Efficient Hybrid Inline and Out-of-line Deduplication for Backup Storage

Backup storage systems often remove redundancy across backups via inline deduplication, which works by referring duplicate chunks of the latest backup to those of existing backups. However, inline deduplication degrades restore performance of the latest backup due to fragmentation, and complicates deletion of ex- pired backups due to the sharing of data chunks. While out-of-line deduplication addresses the problems by forward-pointing existing duplicate chunks to those of the latest backup, it introduces additional I/Os of writing and removing duplicate chunks. We design and implement RevDedup, an efficient hybrid inline and out-of-line deduplication system for backup storage. It applies coarse-grained inline deduplication to remove duplicates of the latest backup, and then fine-grained out-of-line reverse deduplication to remove duplicates from older backups. Our reverse deduplication design limits the I/O overhead and prepares for efficient deletion of expired backups. Through extensive testbed experiments using synthetic and real-world datasets, we show that RevDedup can bring high performance to the backup, restore, and deletion operations, while maintaining high storage efficiency comparable to conventional inline deduplication.

==> background.tex <==
\section{Basics}
\label{sec:background}

%We overview the basics of backup operations, and motivate how inline
%deduplication can hamper the restore and reclamation performance of backup
%systems.  We also review related work on deduplication.  

%Deduplication is known to improve storage efficiency of backup systems by
%identifying duplicate data and keeping only the first copy. However, the
%traditional deduplication approach is not optimized for backup workload and
%designing a backup system making use of deduplication is challenging. In this
%section, we first discuss the design challenges in utilizing deduplication in
%backup systems, afterwards, we review several related works in different
%aspects.

\subsection{Backups}
\label{subsec:backups}

{\em Backups} are copies of primary data snapshotted from client systems or
applications, and can be represented in the form of {\tt tar} files or VM disk
images (e.g., {\tt qcow2}, {\tt vmdk}, etc.).  They are regularly created by a
backup system, either as daily incremental backups or weekly full backups.
Backup data is organized into {\em containers} as the units of storage and
read/write requests. Each container is typically of size on the order of
megabytes.  Backup systems copy the containers to storage devices, which are
mostly disk-based nowadays. 

We define a {\em series} as the sequence of backups snapshotted from the same
client instance at different times.  Each backup series has a retention period
\cite{wallace12}, which defines how long a backup is kept in storage.  We
define a {\em retention window} that specifies a set of recent backups that
need to be kept in storage.  The retention window slides over time to cover
the latest backup.  The earliest backup stored in the system then expires.
The backup system later deletes the expired backups and reclaims storage
space.   Note that the retention window length may vary across different
backup series. 

\subsection{Inline vs. Out-of-line Deduplication}
\label{subsec:vs}

Deduplication exploits content similarity to eliminate redundant data.
Conventional inline deduplication approaches treat data as a stream of
fixed-size or variable-size {\em chunks}, typically of size 4-8KB each
\cite{zhu08,guo11}.  Each chunk is identified by a {\em fingerprint} computed
by a cryptographic hash (e.g., MD5, SHA-1) of its content.  Two chunks are
said to be identical if their fingerprints are the same. We assume that the
probability that two different chunks have fingerprint collisions is
negligible \cite{black06}.

Today's production backup systems \cite{zhu08,wallace12,lillibridge13} mainly
implement {\em inline deduplication}, which eliminates redundancy on the write
path.  However, it poses several fundamental challenges to the basic
operations of backup systems, including backup, restore, and deletion: 
%
\begin{itemize}
\item
{\em Backup:}  Inline deduplication avoids writing duplicate data, and hence
in general achieves faster backup performance than without deduplication.
However, the backup performance is also determined by metadata operations,
including fingerprint computations, fingerprint lookups, and metadata updates.
The number of fingerprints increases proportionally with the raw storage size.
Thus, keeping all fingerprints and other indexing metadata in main memory is
infeasible.  Instead, some indexing metadata must be kept on disk, but this
incurs disk accesses for metadata lookups and degrades backup performance.
\item
{\em Restore:}  Inline deduplication stores references that refer to the
identical chunks that are already stored in other containers. This leads to 
{\em fragmentation} \cite{rhea08,kaczmarczyk12,nam12,lillibridge13}.
Restoring backups will incur disk seeks to containers, and this degrades
restore performance.
%The degradation due to disk seeks can be illustrated via simple calculation.
%Consider a generic 7200~RPM 3.5-inch SATA harddisk with an average seek time
%of 8.5ms \cite{seagate}.  With only 60 disk seeks per second on the read
%path, the effective read bandwidth will drop by at least 50\%, since more
%than half of the time is spent on disk seeks. 
Furthermore, data fragmentation becomes worse for newer backups, which can
refer to more duplicate chunks in older backups and have chunks more spread
out.  The gradual degradation is undesirable for backup systems, since the new
backups are more likely to be restored during disaster recovery.  A lower
restore throughput of the latest backup implies a longer system downtime. 
%Therefore, the fragmentation should be taken into account especially on most
%recent backup should be taken into account.
\item
{\em Deletion:}  
%Deletion of expired backups cannot be directly performed when inline
%deduplication is enabled since old backups may be shared by non-expired
%backups.  
Inline deduplication systems often handle deletion through a mark-and-sweep
approach: in the mark phase, all chunks are scanned and any unreferenced
chunks are marked for removal; in the sweep phase, all marked chunks are freed
from disk in the background.   However, the mark phase needs to search for
unreferenced chunks through all containers, thereby incurring significant
I/Os.  Also, removed chunks become ``holes'' in a container and lead to {\em
disk fragmentation}.  If variable-size chunking is used, then the space of the
removed chunks cannot be reused for larger chunks.  To reclaim the free space
from removed chunks, containers need to be compacted or merged
\cite{strzelczak13}, but this again incurs heavy I/Os. 
\end{itemize}

{\em Out-of-line deduplication} first writes all data to disk and then
removes duplicate chunks from disk.  It addresses some aforementioned issues
of inline deduplication.  For example, it can reduce the disk overhead of
metadata lookups via batch processing \cite{lillibridge09}.  It also mitigates
data fragmentation and preserves restore performance of the new backups using
forward-pointing deduplication, i.e.,  removing duplicate chunks of old
backups and referring them to the chunks of new backups \cite{kaczmarczyk12}.
The forward-pointing approach also facilitates the deletion of old backups,
since their chunks are no longer shared by new backups.  However,
out-of-line deduplication has two major drawbacks.  First, it introduces
extra I/Os of writing and removing redundant data.  It generally gives worse
backup performance than inline deduplication because it writes redundant data. 
Second, it requires extra storage space to store redundant data before the
redundancy is removed. 

%-- obsolete --

%In deduplication systems, data blocks are identified by a fingerprint generated by taking a cryptographic hash (e.g. SHA-1) of the content and two identical data blocks would produce the same fingerprint. Therefore, deduplication systems maintain a fingerprint index recording all data blocks stored. During subsequent backups, fingerprints of incoming blocks are filtered against the index to identify any duplicates. The index would expand with stored data, considering a storage with 100TB unique data with 8KB segment size and each fingerprint takes up 20Bytes, the full index would take up 250GB space and impossible to be in-memory. Storing this index on-disk would incur disk I/O during the filtering phase and as fingerprints are considered random, caching could hardly be done.  As a result, the on-disk lookup could become the bottleneck in performing deduplication. DDFS \cite{zhu08} and Foundation \cite{rhea08} use Bloom Filter \cite{bloom70} to filter index lookup. Meister {\em et al.} \cite{meister13} find that Bloom Filter could filter much on-disk lookup where the system is new as most incoming data are unique and could be identified with the small in-memory bloom filter, it only has small effect in subsequent backups are most incoming data are duplicates, to check duplicates, bloom filter require a verification with the full index in case of false positive result. Therefore, it does not help in relieving the disk bottleneck with backup storage which duplicate data is expected to be the dominate case. DDFS and other studies \cite{lillibridge09, bhagwat09, kruus10, guo11, xia11, simha13} exploit workload characteristics such as locality and similarity of data to improve the fingerprint caching and reduce memory usage of indexing by utilizing sampling.  Kruss {\em et al.} proposes a bimodal chunking method such that a small chunk size is used in limited regions of transition from duplicate to non-duplicate data and large chunks are used for elsewhere such that the fingerprint index could keep small with the large average chunk size and the deduplication ratio could be maintained with the small chunks in transition regions.

%Deduplication destroys the sequential layout of backup on disk as blocks of a backup could scatter across prior backups. The fragmentation problem is worse in later backups as the constituent blocks could reference to more old backups and the restore throughput would keep decreasing across the timeline as discussed in previous section \ref{subsec:challenges}. Kaczmarczyk {\em et al.} \cite{kaczmarczyk12} improve restore performance by selectively rewriting data that benefits reads. Nam {\em et al.} \cite{nam12} measure the fragmentation impact given the input workload and perform deduplication selectively.  Lillibridge {\em et al.} \cite{lillibridge09} limit the chunk scattering by imposing a container capping and improve the restore performance by forward assembly area. iDedup \cite{srinivasan12} only deduplicates sequence of duplicate blocks instead of every single duplicates so as to reduce the latency brought by frequent disk seeks. While these works have proposed different measures to limit the fragmentation, we are going to take a different approach to shift the fragmentation from new backups to old backups such that restore throughput of most recent are optimized.  

